Numerical Analysis of the Screening Current-Induced Magnetic Field in the HTS Insert Dipole Magnet Feather-M2.1-2

Screening currents are field-induced dynamic phenomena which occur in superconducting materials, leading to persistent magnetization. Such currents are of importance in ReBCO tapes, where the large size of the superconducting filaments gives rise to strong magnetization phenomena. In consequence, superconducting accelerator magnets based on ReBCO tapes might experience a relevant degradation of the magnetic field quality in the magnet aperture, eventually leading to particle beam instabilities. Thus, persistent magnetization phenomena need to be accurately evaluated. In this paper, the 2D finite element model of the Feather-M2.1-2 magnet is presented. The model is used to analyze the influence of the screening current-induced magnetic field on the field quality in the magnet aperture. The model relies on a coupled field formulation for eddy current problems in time-domain. The formulation is introduced and verified against theoretical references. Then, the numerical model of the Feather-M2.1-2 magnet is detailed, highlighting the key assumptions and simplifications. The numerical results are discussed and validated with available magnetic measurements. A satisfactory agreement is found, showing the capability of the numerical tool in providing accurate analysis of the dynamic behavior of the Feather-M2.1-2 magnet.

==> Section/SEC99_CodeGraveyard.tex <==
%*************************************************%
%* FORMULATION ***********************************%
%*************************************************%
\subsection{Formulation of the Field Problem}
    \label{SEC_FormulationOfTheFieldProblem}
% 
%------------------------------% 
\begin{figure}[tb]
  \centering
	\includegraphics[width=8.0cm]{Figure/FIG_DomainDecomposition.PNG}
	\caption{}
	\label{FIG_DomainDecomposition}
    % \vskip -0.25cm
\end{figure}
%------------------------------%    
The computational domain $\SCA{\RMOmega}$ representing the superconducting magnet is decomposed into the source and source-free regions $\SCAl{\RMOmega}{\RM{H}}$ and $\SCAl{\RMOmega}{\RM{A}}$, such that $\SCAl{\BAR{\RMOmega}}{\RM{H}}\cup\SCAl{\BAR{\RMOmega}}{\RM{A}}=\SCA{\BAR{\RMOmega}}$. The source region corresponds to the coil containing the superconducting materials. The source-free region contains the remaining of the magnet, consisting of the iron yoke, the mechanical supports, and the air region. Such decomposition allows to assume a constant magnetic permeability $\ITmu$ in $\SCAl{\RMOmega}{\RM{H}}$, whereas a nonlinear dependency from the magnetic field $\VEC{B}$ is considered for the iron yoke in $\SCAl{\RMOmega}{\RM{A}}$, as $\ITmu(\VEC{B})$. 

Thanks to the domain decomposition, the field problem is solved under magnetoquasistatic assumptions for the reduced magnetic vector potential $\VECu{A}{\star}$~\cite{emson1983optimal} in $\SCAl{\RMOmega}{\RM{A}}$, and for the magnetic field strength $\VEC{H}$ in $\SCAl{\RMOmega}{\RM{H}}$. The formulation reads
%------------------------------% 
    \begin{align}
        \label{EQstrongAampereMaxwell}
            \EQstrongAampereMaxwell{}\ \text{in}\ \SCAl{\RMOmega}{\RM{A}}, \\
        \label{EQstrongHfaraday}
            \EQstrongHfaraday{}\ \text{in}\ \SCAl{\RMOmega}{\RM{H}}, \\ 
        \label{EQconstraintIsource}
            \EQconstraintIsource{} &= \SCAl{i}{\RM{s}}, 
    \end{align}
%------------------------------% 
where $\VEC{\ITchi}$ is a voltage distribution function~\cite{rodriguez2008voltage,schops2013winding}, $\SCAl{u}{\RM{s}}$ is the source voltage treated as an algebraic unknown, and $\SCAl{i}{\RM{s}}$ is the source current which is imposed via a constraint equation (i.e., a Lagrange multiplier). The fields $\VECu{A}{\star}$ and $\VEC{H}$ are linked via continuity conditions at the interface of the domains. In particular, the continuity of the normal component of the magnetic field $\VECl{B}{\RM{n}}$ and the current density $\VECl{J}{\RM{n}}$, and the tangential component of the magnetic field strength $\VECl{H}{\RM{t}}$ and electric field strength $\VECl{E}{\RM{t}}$ are imposed. This ensures the consistency of the overall field solution.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* OLD INTRODUCTION ******************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CONTENTS:
% 1. HTS technology in accelerators
% 2. Where HTS technology stands at the moment
% 3. Need for high quality fields
% 4. Issue with persistent currents
% 5. Importance of high-accuracy numerical methods in designing HTS magnets
% 4. Gap sentence: what is new?
% 5. Objective: what did we do in our work?
% 6. How did we reach our objective?
% 7. Short summary

% \section{Introduction} 
%     \label{SEC_Introduction}


% High Temperature Superconducting (HTS) materials are a promising technology for accelerator magnets in particle accelerators. In particular, superconducting tapes based on {R}e{BCO} compounds~\cite{wu1987superconductivity} show a critical temperature of $\SI{93}{\kelvin}$ and an estimated upper critical field of $\SI{140}{\tesla}$~\cite{golovashkin1991low}. These properties are about one order of magnitude higher than in traditional Low Temperature Superconducting (LTS) materials, such as $\RM{Nb{\HYPHEN}Ti}$ or $\RM{Nb_{3}Sn}$~\cite{wilson1983superconducting}. Thus, HTS materials might be exploited in building accelerator magnets with higher magnetic fields and higher thermal margins~\cite{van2016high}. A remarkable milestone in this direction was recently achieved by the {E}u{CARD}-2 project~\cite{rossi2015eucard}, which led to the construction of the HTS accelerator dipole insert-magnet \FEATHER.1$\HYPHEN$M2~\cite{kirby2014accelerator,van2014study}. This demonstrator magnet is designed to be operated inside a background magnetic field, produced for example by the {FRESCA2} dipole magnet~\cite{milanese2011design,ferracin2013development}. The magneto-thermal behavior of the insert was recently tested in a stand-alone configuration~\cite{van2018powering}, and the magnetic field quality was measured~\cite{petrone2018measurement}.

% One of the key requirements for accelerator magnets is to produce high-quality magnetic fields in their magnet aperture (see e.g.,~\cite{bruning2004lhc}), as field imperfections can lead to particle beam instabilities~\cite{shi2000collective}. Therefore, the current density distribution within the superconductor should be as uniform as possible. Conversely, HTS tapes behave as wide and anisotropic mono-filaments, allowing for strong screening currents in the dynamic regime which prevent an homogeneous current density distribution, \CORRI{deteriorating the field quality~\cite{uglietti2010measurements,yanagisawa2010magnitude,amemiya2015magnetisation,dilasser2016experimental,wang2016screening,fazilleau2018screening,noguchi2019simple}}. Such currents do not decay as they flow in a superconducting material, producing a persistent magnetization. The magnetization is more relevant at low-field, where screening currents are typically much higher than the transport current. Attempts in limiting persistent magnetization phenomena by tape striation~\cite{nast2014influence} or tape-field alignment~\cite{van2016measurement} are not fully satisfactory. \CORRI{Thus, persistent magnetization phenomena need to be carefully evaluated, and possibly predicted by means of numerical models, as they may limit the use of HTS technology in accelerator magnets.} 

% % Numerical models can play a determinant role in providing accurate simulations of these magnetic phenomena in superconducting magnets.

% In this paper, we present the time domain analysis of \CORRI{the screening current-induced magnetic field} in the \FEATHER magnet. A dedicated 2D numerical model is developed using the finite element method (FEM, e.g,~\cite{zienkiewicz2005finite}). The model implements a coupled $\VEC{A}\HYPHEN\VEC{H}$ field formulation~\cite{biro1999edge} for HTS materials~\cite{dular2019finite}, extended to the simulation of HTS magnets~\cite{bortot2020coupled}. \CORRI{The model implements a domain decomposition strategy, solving for the magnetic field strength $\VEC{H}$ in the superconducting regions, and for the magnetic vector potential $\VEC{A}$ in the normal conducting and nonconducting regions. Thus,} the electrodynamic phenomena occurring within the superconducting coil are taken into account by solving a time-domain, eddy current, \CORRI{coupled} problem. The model provides an accurate prediction of persistent currents and their influence on the magnetic field quality. Moreover, simulations resolve the current density distribution within the superconductor, which is crucial for the determination and understanding of the Joule losses and the Lorentz forces in the coil. The model is verified against theoretical results, and cross-checked with magnetic measurements. In particular, the net contribution of the persistent magnetization on the magnetic field quality is discussed. 

% The paper is structured as follows. In Section II, the coupled field formulation is described and verified against theoretical references. Section III illustrates the FEM model of the \FEATHER magnet, highlighting assumptions and simplifications. The field quality comparison between numerical and measurement results is presented in Section IV, followed by the discussion of the results and conclusions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* MAGNETIC FIELD QUALITY AFTER STEFAN ***********%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CONTENTS:   
% Principles: How it is given, and why
% How it is measured
% How it is simulated
% 

% \section{Magnetic Field Quality}
%     \label{SEC_Measurement}
% The  magnetic field quality in accelerator magnets is defined as the set of Fourier coefficients, known also as field harmonics or multipole coefficients. The coefficients are derived from the general solution of the field problem in the source-free magnet aperture, which is given by the Laplace equation $\GRAD^{2}\VEC{A}$. Since the field is assumed to be constant in time and uniform in the $z$-direction (the longitudinal magnet axis), the general solution (e.g.~\cite{russenschuck2011field}) can be expressed as
% %% spacer_For_Empty_Line  
% \begin{equation}
%     \label{solll} 
%      \SCAl{A}{\RM{z}}(r,\ITvarphi)= 
%      \sum_{n=1}^{\infty} r^n
%      (\SCAl{\cal{A}}{n} \sin n\ITvarphi + \SCAl{\cal{B}}{n} \cos n\ITvarphi). 
% \end{equation}
% %% spacer_For_Empty_Line 
% where $\SCAl{A}{\RM{z}}$ is the longitudinal component of the magnetic vector potential, $\SCAl{\cal{A}}{n}$ and $\SCAl{\cal{B}}{n}$ are the multipole coefficients, and $(r,\ITvarphi,z)$ are spatial coordinates in a cylindrical reference system. The field components are obtained from~\eqref{solll} as
% %% spacer_For_Empty_Line 
% \begin{align}
%     \label{br} 
%     \SCAl{B}{r}(r,\ITvarphi) &= 
%     % \frac{1}{r} \frac{\partial A_z}{\partial \ITvarphi} =  
%      \sum_{n=1}^{\infty} n r^{n-1} ( \SCAl{\cal{A}}{n} \cos n\ITvarphi
%     - \SCAl{\cal{B}}{n} \sin n\ITvarphi ) , \\
%     \label{bf} 
%     \SCAl{B}{\ITvarphi}(r,\ITvarphi) &= 
%     % - \frac{\partial A_z}{\partial r} =
%     - \sum_{n=1}^{\infty} n r^{n-1} (\SCAl{\cal{A}}{n} \sin n\ITvarphi +
%     \SCAl{\cal{B}}{n} \cos n\ITvarphi ).
% \end{align}
% %% spacer_For_Empty_Line 
% The index $n$ represents solutions of the Laplace equation which can be associated to field distributions generated by ideal magnet geometries. As example, $n$ = 1,2,3 correspond to the dipole, quadrupole, and sextupole field distributions. Once the radial field component~\eqref{br} is known at a reference radius $r = \SCAl{r}{0}$ (either by measurements or simulations), the normal and skew multipole coefficients $\SCAl{B}{n}$ and $\SCAl{A}{n}$ are obtained for $n=1,2,3,\ldots$, as  
% %
% \begin{align}
%     \SCAl{A}{n}(\SCAl{r}{0}) &= 
%     \frac{1}{\pi} \int_{0}^{2\pi}
%     \SCAl{B}{r}(\SCAl{r}{0},\ITvarphi) 
%     \cos n\ITvarphi\ {d}\ITvarphi, \\
%     % \ n=1,2,3,\ldots , \\
%     \SCAl{B}{n}(\SCAl{r}{0}) &= 
%     \frac{1}{\pi} \int_{0}^{2\pi} 
%     \SCAl{B}{r}(\SCAl{r}{0},\ITvarphi) 
%     \sin n\ITvarphi \ {d}\ITvarphi.
%     % \ n=1,2,3,\ldots . 
% \end{align}
% %% spacer_For_Empty_Line 
% The radius $\SCAl{r}{0}$ is usually chosen as 2/3 of the magnet aperture. The coefficients are often combined in the complex notation $C_n(\SCAl{r}{0})=\SCAl{B}{n}(\SCAl{r}{0})+i~\SCAl{A}{n}(\SCAl{r}{0})$ as the skew and normal pairs are orthogonal to each other. Moreover, the coefficients are typically normalized with respect to the main field component $\SCAl{B}{\RM{N}} (\SCAl{r}{0})$, and denoted as $\SCAl{b}{n}$ and $\SCAl{a}{n}$. Thus, the field quality is quantified as a relative error $\SCAl{c}{n}$, for $n=1,2,3,\ldots$, as
% %% spacer_For_Empty_Line 
% \begin{equation}
% c_n(\SCAl{r}{0}) = \SCAl{b}{n}(\SCAl{r}{0}) + i \SCAl{a}{n}(\SCAl{r}{0}) = 10^4 \frac{C_n(\SCAl{r}{0})}{\SCAl{B}{\RM{N}}},
% \label{eq:eqH7}  
% \end{equation} 
% %% spacer_For_Empty_Line 
% and given in $\SI{1e-4}{}$ units with respect to $\SCAl{B}{\RM{N}}$ at the reference radius $\SCAl{r}{0}$.

% \subsection{Rotating-Coil Magnetometers}
% Rotating-coil magnetometers,  also known as harmonic coils, are electromagnetic transducers for measuring the $\SCAl{B}{n}$ and $\SCAl{A}{n}$ field multipoles.
% Rotating the coil shaft in the magnet aperture, parallel to the magnetic axis of the magnet, the change of flux linkage induces, by Faraday\'{}s law, a voltage signal on the coil terminal. By integrating in time the voltage signal, the flux linkage is obtained and given as a function of the series expansion of the radial field~\cite{russenschuck2011field}. The mean surface and the mean radius of the coil are calibrated in a dipole and quadrupole reference magnet. 

% \subsection{Measurement Setup}
% Encouraged by the results obtained from the flux sensors presented in~\cite{petrone2018measurement}, a dedicated rotating-coil magnetometer was developed and employed to test the Feather2 magnet in the variable temperature cryostat at CERN.
% %
% The constructed coil shaft is composed of a chain of five Printed-Circuit Boards (PCBs), ($\SI{200}{mm}$ in length and~$\SI{35}{mm}$ in width), that span the entire magnet length including the fringe-field areas. Every PCB board contains three coils mounted radially, with an active surface of~$\SI{0.1817}{m^{2}}$. For the magnetic-field harmonics, the measurement sensitivity improves by connecting two coils in anti series; for the dipole magnet measurement the external coil minus the central coil. {CERN} proprietary digital cards integrate the induced voltages in the coils rotating at a frequency of~$\SI{2}{Hz}$. 
% %
% In this paper, the measurement results are taken from the longitudinal center of the magnet (the central element of the rotating shaft of 200 mm in length), delivering a measurement precision of a magnetic-field harmonic of $\pm0.05$ units.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* OLD RESULTS ***********************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The net contribution of the persistent currents on the magnetic field quality is evaluated as follows. With respect to the current profile shown in Fig.~\ref{FIG_NormalizedStaircase}, each plateau appears twice for the same current, once during the ramp-up and again during the ramp-down. \CORRI{By subtracting the field quality evaluations obtained at the same current, it is possible to eliminate the field error contributions from both, the not-ideal geometry of the coil, and the iron saturation, which are the same for both the evaluations.} The contribution of the iron hysteresis is discussed separately (see Sec.~\ref{SUBSEC_IronHysteresis}).

% The simulations and measurements are given in Fig.~\ref{FIG_FieldQualityPersistentCurrent} with solid lines and markers. The layout is the same as before for Fig.~\ref{FIG_FieldQuality}. The simulation results are shown for an ${n}$-value of 20. The rows show from top to bottom the variation in units for the multipoles $\SCAl{b}{\RM{1}}$, $\SCAl{b}{\RM{3}}$, $\SCAl{b}{\RM{5}}$ and $\SCAl{b}{\RM{7}}$, as a function of the supply current. The columns separate the results by the operational temperature of the magnet, namely 4.5, 9, 25, and $\SI{68}{\kelvin}$. 

% It is worth noting that the graph show the width of the magnetization loops from Fig.~\ref{FIG_FieldQuality}. The shaded area represents the envelope of the parametric solutions obtained by varying the ${n}$-value of the power-law index between 4 and 30.

% The contribution of the persistent currents does not exceed twenty units for $\SCAl{b}{\RM{1}}$ and $\SCAl{b}{\RM{3}}$, two units for $\SCAl{b}{\RM{5}}$ and one unit for $\SCAl{b}{\RM{7}}$. The trend is generally monotone, showing the multipoles decreasing as the current increases, and vanishing as the current reaches its peak value. The $\SCAl{b}{\RM{1}}$ coefficient is an exception, as it has a peak around $\SI{3.5}{\kilo\ampere}$, when the pole of the iron yoke saturates.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* OLD MAGNETIC MEASUREMENT PART *****************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Magnetic Measurements}
%     \label{SEC_Measurement}
% %% CARLO
% \subsection{Principles}
% Magnetic field quality in the aperture of accelerator magnets is commonly described by a set of Fourier coefficients, known to the magnet design community as field harmonics or multipole coefficients. The method used for the calculation of field harmonics is based on finding a general solution that satisfies the Laplace equation in a suitable coordinate system. The integration in the general solution, obtained with the separation of variables technique, are then determined by comparison with the boundary values. %
% Starting from the vector potential that satisfies the Laplace equation, $\GRAD^{2}\SCAl{A}{\RM{z}}=0$, and considering the magnet aperture as the problem domain, a general solution can be found
% %% spacer_For_Empty_Line  
% \begin{equation}
%     \label{solll} 
%      \SCAl{A}{\RM{z}}(r,\ITvarphi)= 
%      \sum_{n=1}^{\infty} r^n
%      (\SCAl{\cal{A}}{n} \sin n\ITvarphi + \SCAl{\cal{B}}{n} \cos n\ITvarphi). 
% \end{equation}
% %% spacer_For_Empty_Line 
% The field components can then be derived from $\SCAl{A}{\RM{z}}$~\cite{russenschuck2011field}, as
% %% spacer_For_Empty_Line 
% \begin{align}
%     \label{br} 
%     \SCAl{B}{r}(r,\ITvarphi) &= 
%     % \frac{1}{r} \frac{\partial A_z}{\partial \ITvarphi} =  
%     +\sum_{n=1}^{\infty} n r^{n-1} ( \SCAl{\cal{A}}{n} \cos n\ITvarphi
%     - \SCAl{\cal{B}}{n} \sin n\ITvarphi ) , \\
%     \label{bf} 
%     \SCAl{B}{\ITvarphi}(r,\ITvarphi) &= 
%     % - \frac{\partial A_z}{\partial r} =
%     - \sum_{n=1}^{\infty} n r^{n-1} (\SCAl{\cal{A}}{n} \sin n\ITvarphi +
%     \SCAl{\cal{B}}{n} \cos n\ITvarphi ), 
% \end{align}
% %% spacer_For_Empty_Line 
% Each value of the integer $n$ in the solution of the Laplace equation corresponding to a specific flux distribution
% generated by ideal magnet geometries. The three lowest values, $n$ = 1,2,3 correspond to the dipole, quadrupole, and sextupole flux
% density distributions. 
% %
% Assuming that the radial component of the magnetic field in Eq.~(\ref{br}) is measured or calculated at a reference radius $r = \SCAl{r}{0}$ as a function of the angular position $\ITvarphi$, the Fourier series expansion of the obtained radial field components is~\cite{russenschuck2011field}
% %% spacer_For_Empty_Line 
% \begin{equation}
%   \label{Four1} 
%     \SCAl{B}{r}(\SCAl{r}{0},\ITvarphi) = 
%     \sum_{n=1}^{\infty} ( \SCAl{B}{n}(\SCAl{r}{0}) \sin n\ITvarphi 
%     + \SCAl{A}{n}(\SCAl{r}{0}) \cos n\ITvarphi ),  
% \end{equation}
% %% spacer_For_Empty_Line 
% where for $n=1,2,3,\ldots$,
% %
% \begin{align}
%     \SCAl{A}{n}(\SCAl{r}{0}) &= 
%     \frac{1}{\pi} \int_{0}^{2\pi}
%     \SCAl{B}{r}(\SCAl{r}{0},\ITvarphi) 
%     \cos n\ITvarphi\ {d}\ITvarphi, \\
%     % \ n=1,2,3,\ldots , \\
%     \SCAl{B}{n}(\SCAl{r}{0}) &= 
%     \frac{1}{\pi} \int_{0}^{2\pi} 
%     \SCAl{B}{r}(\SCAl{r}{0},\ITvarphi) 
%     \sin n\ITvarphi \ {d}\ITvarphi.
%     % \ n=1,2,3,\ldots . 
% \end{align}
% %% spacer_For_Empty_Line 
% It is common practice to normalize the multipole coefficients with respect to the main field component\footnote{This is $\SCAl{B}{1}$ for the dipole, $\SCAl{B}{2}$ for the quadrupole, and so on.} $\SCAl{B}{\RM{N}} (\SCAl{r}{0})$, denoted in lowercase letters, expressed in a reference frame where the main skew component is zero. In case of the radial field component, this yields
% %% spacer_For_Empty_Line 
% \begin{equation}
%     \label{radharmonic}
%     \SCAl{B}{r}(r,\ITvarphi) =  \SCAl{B}{\RM{N}} \sum_{n=1}^{\infty} \!
%     \left(\frac{r}{\SCAl{r}{0}}\right)^{n-N} (\SCAl{B}{n} (\SCAl{r}{0}) \sin n\ITvarphi + \SCAl{A}{n}
%     (\SCAl{r}{0}) \cos n\ITvarphi ). 
% \end{equation}
% %% spacer_For_Empty_Line 
% Applying the following trigonometric 
% functions, $(\cos \ITvarphi + i \sin \ITvarphi)^n = (e^{i\ITvarphi})^n = e^{in\ITvarphi} = \cos n\ITvarphi + i \sin n\ITvarphi$, $n \in \mathbb{Z}$, the magnetic field in Cartesian coordinates components can be expressed as:
% %% spacer_For_Empty_Line 
% \begin{align}
%     \label{fieldcomponent} 
%     \SCAl{B}{\RM{x}}(r,\ITvarphi) = &
%     \sum_{n=1}^{\infty}
%     \left(\frac{r}{\SCAl{r}{0}}\right)^{n-1} \! 
%     (\SCAl{B}{n} (\SCAl{r}{0}) \sin  (n-1) \ITvarphi + \SCAl{A}{n}
%     (\SCAl{r}{0}) \cos (n-1) \ITvarphi )  \\  
%     \label{radcoil4}
%     \SCAl{B}{\RM{y}} (r,\ITvarphi) = &
%     \sum_{n=1}^{\infty} \!
%     \left(\frac{r}{\SCAl{r}{0}}\right)^{n-1} \!
%     (\SCAl{B}{n} (\SCAl{r}{0}) \cos (n-1) \ITvarphi - \SCAl{A}{n}
%     (\SCAl{r}{0}) \sin (n-1) \ITvarphi) 
% \end{align}
% %% spacer_For_Empty_Line 
% where the normal and skew multipole coefficients $\SCAl{B}{n} (\SCAl{r}{0}),
% \SCAl{A}{n} (\SCAl{r}{0})$ are given in Tesla at a reference radius $\SCAl{r}{0}$. They are often combined in the complex notation $C_n(\SCAl{r}{0})=\SCAl{B}{n}(\SCAl{r}{0})+i~\SCAl{A}{n}(\SCAl{r}{0})$. By definition for accelerator magnets, the normal components indicate a vertical field in the horizontal plane while the skew terms indicate an horizontal field. In Fig.~\ref{fig:dipolequadrupooleLineFileds}, the field lines for normal and skew dipoles $(\SCAl{B}{1}, \SCAl{A}{1})$ and quadrupoles $(\SCAl{B}{2}, \SCAl{A}{2})$ are shown.
% %% spacer_For_Empty_Line 

% \subsection{Rotating Coil}
% Multipole coefficients, from different measurement devices for example, must be compared at the same reference radius $\SCAl{r}{0}$. The reference radius $\SCAl{r}{0}$ is an important concept for accelerator magnets and it is usually chosen as 2/3 of the magnet aperture.  
% %% spacer_For_Empty_Line 
% By choosing a complex plane $(x,y)$, the harmonic can be expressed in terms of the complex variable $z=x+iy$ \cite{A.Jain:CAS1997_2}
% %% spacer_For_Empty_Line 
% \begin{equation}
%     \SCA{B}(z)= 
%     \SCAl{B}{\RM{y}}(z) + i \SCAl{B}{\RM{x}}(z) = 
%     \sum_{n=1}^{\infty} {C_n(z) \left(\frac{z}{\SCAl{r}{0}}\right)^{n-1}}.
% \label{eq:eqH6}  \end{equation}
% %% spacer_For_Empty_Line 
% The field quality, described as relative errors with respect to the main field component $\SCAl{B}{\RM{N}}$ at the reference radius $\SCAl{r}{0}$, is given by
% %% spacer_For_Empty_Line 
% \begin{equation}
% c_n = \SCAl{B}{n} + i \SCAl{A}{n} = 10^4 \frac{C_n}{\SCAl{B}{\RM{N}}}.
% \label{eq:eqH7}  
% \end{equation} 
% %% spacer_For_Empty_Line 
% This is perfectly in accordance with a field magnetic measurement method using rotating coils, as will be described in the next paragraph. Rotating harmonic coils, also known outside from measurement field as search coils or pickup coils, are electromagnetic transducers used for measuring the field harmonics coefficients $\SCAl{B}{n}$ and $\SCAl{A}{n}$.
% %% spacer_For_Empty_Line 
% The physical principle of the coils measurement is based on Lenz\'{}s law: when a conductor loop moves with respect to a magnetic field, a flux variation occurs and a voltage proportional to this flux variation is induced. A flux change inside the coil is achieved either by varying the magnetic field (for example varying the magnet excitation current), or by moving the coil inside the magnetic field. If the sensing coil is made to rotate around the magnet axis, the principle is known as the harmonic coil methods \cite{Walckiers:CAS2009_2}. A change of flux induces, by Faraday\'{}s law, a voltage signal $U$ on the terminal of the coil
% %% spacer_For_Empty_Line 
% \begin{equation}
%     U = -\frac{\RM{d}{\RMPhi}}{\RM{d}{t}}.
%     \label{voltageDerivateFlux} 
% \end{equation}
% %% spacer_For_Empty_Line 
% A magnetic flux measurement by means of the rotating coils thus requires the integration of the voltage induced on the coil 
% %% spacer_For_Empty_Line 
% \begin{equation}
%  \RMPhi = -\int_{t_1}^{t_2}{U \RM{d} t}. 
%  \label{eq:fluxIntegralVoltage} 
% \end{equation}
% Since the field is assumed to be constant in time and uniform in the $z$-direction (the longitudinal magnet axis), the flux linkage through the coil with $N$ turns and area $\SCA{S}$, can be calculated from
% %% spacer_For_Empty_Line 
% \begin{align}
%     \ITPhi (\ITvarphi) &= 
%     N \int_{\SCA{S}}^{}{ \! \VEC{B} \cdot \RM{d} \VEC{a}},
% \label{eq:fluxIntegral}
% \end{align}
% %
% where $\VEC{B}$ is the magnetic field and $\RM{d} \VEC{a}$ is the surface element vector. The units of Eq.(\ref{eq:fluxIntegral}) are $ [ \Phi ] = \text{V} \text{s}  = \text{T} \text{m}^2  = \text{Wb}$.
% %
% The coil is assumed to be perfectly centered in the aperture of a magnet and to rotate rigidly around its axis at the angular velocity $\omega$. Therefore, at time $t$ the search coil will be located at the angular position $\ITvarphi = \omega t + \Theta$, where $\Theta$ is the angle at $t=0$. A positive angle in the reference frame corresponds to a counter-clockwise rotation as shown in Fig.~\ref{fig:chemeCoilAxisAngle}.

% The following equation,
% %
% \begin{equation}
% \SCA{S}  = N  \ell  \int_{r_1}^{r_2}{\RM{d}r} = N \ell (r_2-r_1),
% \label{eq:surfaceIntegral}   
% \end{equation}
% %
% represents the surface for all the turns of a search coil rotating around the axis $r$ (assuming that the windings are infinitely thin) where $\ell$ is the length of the search coil. The angle $\ITvarphi$ describes a rotation of the surface around the axis, with extremities $r_2$ and $r_1$, see Fig. \ref{fig:chemeCoilAxisAngle}.  Therefore, for any angle $\ITvarphi$ the location can be expressed by $ z = x+i y=r e^{i\ITvarphi}. $

% Expressing the magnetic field \textbf{B} in Eq. (\ref{eq:fluxIntegral}) by means of the radial field (\ref{radFieldcoil}) component yields
% %
% \begin{equation}
% \Phi (\ITvarphi) =  \text{Re} \left(N  \ell \int_{r_1}^{r_2}{\vec{B}_r(r,\ITvarphi) \cdot \RM{d} \vec{r}} \right),  
% \label{eq:eqIntegralR1R2}   
% \end{equation}

% and the flux linkage $\Phi (\ITvarphi) $, expressed as a function of the series expansion of the radial field, yields \cite{Russenschuck:Book_2}[MISSING]:
% %
% \begin{align}
% & \Phi (\ITvarphi) = \nonumber \\
% & N \ell  \, \left[  \sum_{n=1}^{\infty}  \frac{\SCAl{r}{0}}{n} 
%  \left(\frac{r_2}{\SCAl{r}{0}}\right)^{n} \! \! (\SCAl{B}{n} (\SCAl{r}{0}) \cos n \varphi_2 + \SCAl{A}{n} (\SCAl{r}{0})
% \sin n \varphi_2)  \right. \nonumber \\
% &  \, \, \left. - \sum_{n=1}^{\infty}  \frac{\SCAl{r}{0}}{n} 
%  \left(\frac{r_1}{\SCAl{r}{0}}\right)^{n} \! \! (\SCAl{B}{n} (\SCAl{r}{0}) \cos n \varphi_1  + \SCAl{A}{n} (\SCAl{r}{0})
% \sin n \varphi_1) \right]. 
% \label{k_prep}
% \end{align}

% The field harmonics are then deduced by exploiting the knowledge of the coil calibration by measuring the flux linkage in reference dipole and quadrupole magnets for the mean surface and the mean radius of the coil, respectively.

% The rotating coil method is nowadays widely used for measuring magnetic field integrated over the coil length, the direction of the main field component with respect to the measuring coil direction, and the axis of a quadrupole or sextupole magnet with respect to the rotation axis of the measuring coil~\cite{Bottura:2000_2}[MISSING]. These measurements are fundamental for accelerator magnets since the beam closed orbit is defined by the residual tilt of the dipole magnets and the quadrupole misalignment~\cite{Bottura:CAS1997_2}[MISSING]. This property is also useful to align the set of measured multipoles in the symmetry axis of the magnet.

% \subsection{Measurement campaign}
% Encouraged by the outcome from the flux sensors presented in~\cite{petrone2018measurement}, a dedicated rotating-coil magnetometer was developed and employed to test the Feather2 magnet in June 2017 in the variable temperature cryostat at CERN. Rotating-coil magnetometers (conductive coils mounted on a rotating shaft) are the standard transducers for measuring the magnetic-field harmonics in accelerator magnets. They are based on Faraday's law, where the induced voltage is proportional to the coil flux linkage.
% %
% The constructed shaft presents a chain of five Printed-Circuit Boards (PCBs), ($\SI{200}{mm}$ in length and~$\SI{35}{mm}$ in width), span the entire magnet length including the fringe-field areas. Every board features three conductive coils mounted radially, with an active surface of~$\SI{0.1817}{m^{2}}$. For the magnetic-field harmonics, the measurement sensitivity improves by connecting two coils in anti series (external coil minus central coil for dipole magnet $A-C$). {CERN} proprietary digital cards integrate the induced voltages over the coils rotating at a frequency of~$\SI{2}{Hz}$. 
% %
% In this paper, the measurement results explored are from the longitudinal center of the magnet (the central element of the rotating shaft), delivering a measurement precision of a magnetic-field harmonic of $\pm0.05$ unit (1 unit is $10^{-4}$ of the main field).

==> Util/UTIL_math.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* LABELLING *************************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% EQ +
%       def 
%       constraint
%       strong
%       weak
%       boundary
%       dirichlet
%       neumann
%       interface
%       discrete
%       mat
%       sys
%           + <optional> coeff
%                + <Variables> (e.g.,A,H,B,T)
%                    + <name>  (e.g. ampereMaxwell)  

% example:
% \EQ + strong + A + ampereMaxwell

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* FORMULATION ***********************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\EQdefJpowerLaw}[0]
    { 
    \SCA{\ITrho}(|\VEC{J}|) =
    \frac{\SCAl{E}{\RM{c}}}{\SCAl{J}{\RM{c}}}
    \left(\frac{|\VEC{J}|}{\SCAl{J}{\RM{c}}}\right)^{{n}-1}
    }
       
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* 3D AH FORM ************************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%* STRONG FORM ------------------------------------

\newcommand{\EQstrongAampereMaxwell}[0]
    { 
    \CURL\ITmu^{-1}\CURL\VECu{A}{\star} 
    + \SCA{\ITsigma}\dxP{t}\VECu{A}{\star} 
    & = 0
    }
   
\newcommand{\EQstrongHfaraday}[0]
    { 
    \CURL\SCA{\ITrho}\CURL\VEC{H} 
    + \dxP{t}\SCA{\ITmu}\VEC{H} 
    - \CURL\VEC{\ITchi}\SCAl{u}{\RM{s}} 
    & = 0
    }
   
\newcommand{\EQconstraintIsource}[0]
    { 
    \int\limits_{\SCAl{\RMOmega}{\RM{H}}}\!\!
    \VEC{\ITchi}\cdot(\CURL\VEC{H})
    \D{\SCA{\RMOmega}} 
    }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* MAGNETIC FIELD QUALITY ************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\EQdefStrongLaplaceAz}[0]
    {
    \SCAl{A}{\RM{z}}(r,\ITvarphi)= 
    \sum_{k=1}^{\infty}{r}^{k}
    (\SCAl{\cal{A}}{k} \sin{k}\ITvarphi + \SCAl{\cal{B}}{k} \cos{k}\ITvarphi)
    }
    
\newcommand{\EQdefStrongLaplaceBr}[0]
    {
    \SCAl{B}{r}(r,\ITvarphi) &= 
    \sum_{k=1}^{\infty}{k}{r}^{k-1} 
    (\SCAl{\cal{A}}{k} \cos{k}\ITvarphi - \SCAl{\cal{B}}{k} \sin{k}\ITvarphi)
    }
    
\newcommand{\EQdefStrongLaplaceBphi}[0]
    {
    \SCAl{B}{\ITvarphi}(r,\ITvarphi) &= 
    - \sum_{k=1}^{\infty}{k}{r}^{k-1} 
    (\SCAl{\cal{A}}{k} \sin{k}\ITvarphi + \SCAl{\cal{B}}{k} \cos{k}\ITvarphi)
    }
    
\newcommand{\EQdefFourierCoeffAk}[0]
    {
    \SCAl{A}{k}(\SCAl{r}{0}) &= 
    \frac{1}{\pi} \int_{0}^{2\pi}
    \SCAl{B}{r}(\SCAl{r}{0},\ITvarphi) 
    \cos{k}\ITvarphi\ {d}\ITvarphi
    }

\newcommand{\EQdefFourierCoeffBk}[0]
    {
    \SCAl{B}{k}(\SCAl{r}{0}) &= 
    \frac{1}{\pi} \int_{0}^{2\pi} 
    \SCAl{B}{r}(\SCAl{r}{0},\ITvarphi) 
    \sin{k}\ITvarphi \ {d}\ITvarphi
    }
    
\newcommand{\EQdefFourierCoeffck}[0]
    {
    \SCAl{c}{k}(\SCAl{r}{0}) = 
    \SCAl{b}{k}(\SCAl{r}{0}) + i \SCAl{a}{k}(\SCAl{r}{0}) 
    = 10^4 \frac{\SCAl{C}{k}(\SCAl{r}{0})}{\SCAl{B}{\RM{K}}}
    }
    
\newcommand{\EQdefFourierTHD}[0]
    {
    \SCAl{F}{\RM{THD}}(\SCAl{r}{0}) = 
    \sqrt{
    \sum_{{k}=1;\ {k}\neq \SCA{K}}^{\infty} 
    \SCAlu{b}{k}{2}(\SCAl{r}{0}) + \SCAlu{a}{k}{2}(\SCAl{r}{0})}
    }
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* VERIFICATION **********************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\EQdefTapeExtFieldLosses}[0]
    {
    \SCAl{w}{\RM{J}} =
    \SCAl{\RMdelta}{\RM{w}}
    \SCAl{J}{\RM{c}}\SCAl{B}{\RM{c}}
    \left(\frac{2}{\SCAl{b}{\RM{p}}}
    \RM{ln}(\RM{cosh}\ \SCAl{b}{\RM{p}})
     -\RM{tanh}\ \SCAl{b}{\RM{p}}\right)
    }
    
\newcommand{\EQdefTapeSelfFieldLosses}[0]
    {
    \SCAl{w}{\RM{J}} =           
    \frac{\SCAl{\ITmu}{0}}{\SCAl{\RMdelta}{\RM{w}}\SCAl{\RMdelta}{\RM{h}}} 
    \SCAlu{I}{\RM{c}}{2}
    \frac{\SCAlu{i}{\RM{p}}{4}}{{6}\ITpi}
    }
    
\newcommand{\EQdefTHDerrorMesh}[0]
    {
    \SCAl{\RMepsilon}{\SCA{\RMDelta{x}}}
    = \frac{|\SCAl{F}{\RM{THD}}-\SCAlu{F}{\RM{THD}}{\SCA{\RMDelta{x}}}|}
    {\SCAl{F}{\RM{THD}}}
    }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* FEATHER-M2 MODEL ******************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\EQdefCorrFactorJc}[0]
    {
    \SCAl{f}{\RM{c}}(\SCA{T}) = 
    \left.\frac{\SCAl{I}{\RM{c,meas}}(\SCA{T})}
    {\SCAl{J}{\RM{c}}
    (\SCAl{B}{\RM{p,coil}}(\SCA{T}),\SCA{T},\SCAl{\RMtheta}{\RM{B}})
   \SCAl{S}{\RM{HTS}}}
    \right\rvert_{\SCAl{\RMtheta}{\RM{B}}=0^{\circ}}
    }
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* MEASUREMENTS **********************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
    
\newcommand{\EQdefRotCoilPhi}[0]
    {
    \RMPhi(t) &= 
    \sum_{k=1}^{\infty}  
    \SCAl{f}{\RM{s}}
    \left[\SCAl{A}{k}(\SCAl{r}{\RM{c0}}) \cos k\ITvarphi
    -\SCAl{B}{k}(\SCAl{r}{\RM{c0}}) \sin k\ITvarphi \right]
    }
    
\newcommand{\EQdefRotCoilSensFactor}[0]
    {
    \SCAl{f}{\RM{s}}(k) &=
    \frac{{2} \SCAl{N}{\RM{c}} \SCAl{l}{\RM{c}} \SCAl{r}{\RM{c0}}}
    {k}
    }

% Version: V 0_0
% Date: 06-01-2020
% Author: lbortot

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* PACKAGES **************************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{textgreek}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* DEFINITIONS ***********************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% FORMAT:
% RM
% IT
% Lowercase first letter name -> lowercase
% Uppercase first letter name -> uppercase

% Low Case Italic 
\newcommand{\ITalpha}[0]{\alpha}
\newcommand{\ITbeta}[0]{\beta}
\newcommand{\ITgamma}[0]{\gamma}
\newcommand{\ITdelta}[0]{\delta}
\newcommand{\ITepsilon}[0]{\epsilon}
\newcommand{\ITvarepsilon}[0]{\varepsilon}
\newcommand{\ITzeta}[0]{\zeta}
\newcommand{\ITeta}[0]{\eta}
\newcommand{\ITtheta}[0]{\theta}
\newcommand{\ITiota}[0]{\iota}
\newcommand{\ITkappa}[0]{\kappa}
\newcommand{\ITlambda}[0]{\lambda}
\newcommand{\ITmu}[0]{\mu}
\newcommand{\ITnu}[0]{\nu}
\newcommand{\ITxi}[0]{\xi}
\newcommand{\ITomicron}[0]{o}
\newcommand{\ITpi}[0]{\pi}
\newcommand{\ITrho}[0]{\rho}
\newcommand{\ITvarrho}[0]{\varrho}
\newcommand{\ITsigma}[0]{\sigma}
\newcommand{\ITtau}[0]{\tau}
\newcommand{\ITupsilon}[0]{\upsilon}
\newcommand{\ITphi}[0]{\phi}
\newcommand{\ITvarphi}[0]{\varphi}
\newcommand{\ITchi}[0]{\chi}
\newcommand{\ITpsi}[0]{\psi}
\newcommand{\ITomega}[0]{\omega}

% Low Case Roman 
\newcommand{\RMalpha}[0]{\textrm{\textalpha}}
\newcommand{\RMbeta}[0]{\textrm{\textbeta}}
\newcommand{\RMgamma}[0]{\textrm{\textgamma}}
\newcommand{\RMdelta}[0]{\textrm{\textdelta}}
\newcommand{\RMepsilon}[0]{\textrm{\textepsilon}}
\newcommand{\RMvarepsilon}[0]{\textrm{\textvarepsilon}}
\newcommand{\RMzeta}[0]{\textrm{\textzeta}}
\newcommand{\RMeta}[0]{\textrm{\texteta}}
\newcommand{\RMtheta}[0]{\textrm{\texttheta}}
\newcommand{\RMiota}[0]{\textrm{\textiota}}
\newcommand{\RMkappa}[0]{\textrm{\textkappa}}
\newcommand{\RMlambda}[0]{\textrm{\textlambda}}
\newcommand{\RMmu}[0]{\textrm{\textmu}}
\newcommand{\RMnu}[0]{\textrm{\textnu}}
\newcommand{\RMxi}[0]{\textrm{\textxi}}
\newcommand{\RMomicron}[0]{\textrm{o}}
\newcommand{\RMpi}[0]{\textrm{\textpi}}
\newcommand{\RMrho}[0]{\textrm{\textrho}}
\newcommand{\RMvarrho}[0]{\textrm{\textvarrho}}
\newcommand{\RMsigma}[0]{\textrm{\textsigma}}
\newcommand{\RMtau}[0]{\textrm{\texttau}}
\newcommand{\RMupsilon}[0]{\textrm{\textupsilon}}
\newcommand{\RMphi}[0]{\textrm{\textphi}}
\newcommand{\RMvarphi}[0]{\textrm{\textvarphi}}
\newcommand{\RMchi}[0]{\textrm{\textchi}}
\newcommand{\RMpsi}[0]{\textrm{\textpsi}}
\newcommand{\RMomega}[0]{\textrm{\textomega}}

% Up Case Italic 
\newcommand{\ITAlpha}[0]{A}
\newcommand{\ITBeta}[0]{B}
\newcommand{\ITGamma}[0]{\mathit{\Gamma}}
\newcommand{\ITDelta}[0]{\mathit{\Delta}}
\newcommand{\ITEpsilon}[0]{E}
\newcommand{\ITZeta}[0]{Z}
\newcommand{\ITEta}[0]{H}
\newcommand{\ITTheta}[0]{\mathit{\Theta}}
\newcommand{\ITIota}[0]{I}
\newcommand{\ITKappa}[0]{K}
\newcommand{\ITLambda}[0]{\mathit{\Lambda}}
\newcommand{\ITMu}[0]{M}
\newcommand{\ITNu}[0]{X}
\newcommand{\ITXi}[0]{\mathit{\Xi}}
\newcommand{\ITOmicron}[0]{O}
\newcommand{\ITPi}[0]{\Pi}
\newcommand{\ITRho}[0]{P}
\newcommand{\ITSigma}[0]{\mathit{\Sigma}}
\newcommand{\ITTau}[0]{T}
\newcommand{\ITUpsilon}[0]{\mathit{\Upsilon}}
\newcommand{\ITPhi}[0]{\mathit{\Phi}}
\newcommand{\ITChi}[0]{X}
\newcommand{\ITPsi}[0]{\mathit{\Psi}}
\newcommand{\ITOmega}[0]{\mathit{\Omega}}

% Up Case Roman 
\newcommand{\RMAlpha}[0]{\mathrm{A}}
\newcommand{\RMBeta}[0]{\mathrm{B}}
\newcommand{\RMGamma}[0]{\Gamma}
\newcommand{\RMDelta}[0]{\Delta}
\newcommand{\RMEpsilon}[0]{\mathrm{E}}
\newcommand{\RMZeta}[0]{\mathrm{Z}}
\newcommand{\RMEta}[0]{\mathrm{H}}
\newcommand{\RMTheta}[0]{\Theta}
\newcommand{\RMIota}[0]{\mathrm{I}}
\newcommand{\RMKappa}[0]{\mathrm{K}}
\newcommand{\RMLambda}[0]{\Lambda}
\newcommand{\RMMu}[0]{\mathrm{M}}
\newcommand{\RMNu}[0]{\mathrm{X}}
\newcommand{\RMXi}[0]{\Xi}
\newcommand{\RMOmicron}[0]{\mathrm{O}}
\newcommand{\RMPi}[0]{\Pi}
\newcommand{\RMRho}[0]{\mathrm{P}}
\newcommand{\RMSigma}[0]{\Sigma}
\newcommand{\RMTau}[0]{\mathrm{T}}
\newcommand{\RMUpsilon}[0]{\Upsilon}
\newcommand{\RMPhi}[0]{\Phi}
\newcommand{\RMChi}[0]{\mathrm{X}}
\newcommand{\RMPsi}[0]{\Psi}
\newcommand{\RMOmega}[0]{\Omega}

% Version: V 0_0
% Date: 06-01-2020
% Author: lbortot

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* PACKAGES **************************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \usepackage{amsmath}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* GENERAL FORMATTING ****************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \mathchardef\HYPHEN="2D
% \newcommand{\BS}     [1] {\bm{#1}}
% \DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}

\newcommand{\HYPHEN} [0] {\operatorname{-}}
\newcommand{\RM}     [1] {\mathrm{#1}}
\newcommand{\BS}     [1] {\boldsymbol{#1}}
\newcommand{\BAR}    [1] {\overline{#1}}
% \newcommand{\OVERBAR} [1] {\mkern7 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* VARIABLES FORMATTING **************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\VEC}   [1] {\protect\vphantom{#1}\smash{\BS{\mathbf{#1}}}}
\newcommand{\VECl}  [2] {\protect\vphantom{#1}\smash{\BS{\mathbf{#1}}}_{#2}}
\newcommand{\VECu}  [2] {\protect\vphantom{#1}\smash{\BS{\mathbf{#1}}}^{#2}}
\newcommand{\VEClu} [3] {\protect\vphantom{#1}\smash{\BS{\mathbf{#1}}}_{#2}^{#3}}

\newcommand{\MAT}   [1] {\protect\vphantom{#1}\smash{\BS{\mathbf{#1}}}}
\newcommand{\MATl}  [2] {\protect\vphantom{#1}\smash{\BS{\mathbf{#1}}}_{#2}}
\newcommand{\MATu}  [2] {\protect\vphantom{#1}\smash{\BS{\mathbf{#1}}}^{#2}}
\newcommand{\MATlu} [3] {\protect\vphantom{#1}\smash{\BS{\mathbf{#1}}}_{#2}^{#3}}

\newcommand{\SCA}   [1] {\protect\vphantom{#1}\smash{\RM{#1}}}
\newcommand{\SCAl}  [2] {\protect\vphantom{#1}\smash{\RM{#1}}_{#2}}
\newcommand{\SCAu}  [2] {\protect\vphantom{#1}\smash{\RM{#1}}^{#2}}
\newcommand{\SCAlu} [3] {\protect\vphantom{#1}\smash{\RM{#1}}_{#2}^{#3}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* VECTOR CALCULUS OPERATORS *********************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\LAPL} [0] {\Delta}
\newcommand{\GRAD} [0] {\nabla}
\newcommand{\DIV}  [0] {\nabla\cdot}
\newcommand{\CURL} [0] {\nabla\times}

% Traces
\newcommand{\LAPLTANG} [0] {\SCAl{\Delta}{\RM{t}}}
\newcommand{\GRADTANG} [0] {\SCAl{\nabla}{\RM{t}}}
\newcommand{\DIVTANG}  [0] {\SCAl{\nabla}{\RM{t}}\cdot}
\newcommand{\CURLTANG} [0] {\SCAl{\nabla}{\RM{t}}\times}
\newcommand{\LAPLNORM} [0] {\SCAl{\Delta}{\RM{n}}}
\newcommand{\GRADNORM} [0] {\SCAl{\nabla}{\RM{n}}}
\newcommand{\DIVNORM}  [0] {\SCAl{\nabla}{\RM{n}}\cdot}
\newcommand{\CURLNORM} [0] {\SCAl{\nabla}{\RM{n}}\times}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* DIFFERENTIAL OPERATORS ************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\D}     [1] {\!\mathop{}\mathrm{d}{#1}}
\newcommand{\dxP}   [1] {\partial_{#1}}
\newcommand{\dx}    [1] {\!\mathrm{\frac{d}{d{#1}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* ALGEBRAIC OPERATORS ***************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TRANS} [0] {\mkern 1mu\top}

==> Util/UTIL_mathVariables.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* CONSTANTS *************************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\MUZERO}      [0] {\ITmu_{\RM{0}}}
\newcommand{\EPSILONZERO} [0] {\ITvarepsilon_{\RM{0}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* DOMAIN DECOMPOSITION **************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% GLOBAL DOMAIN 
% Volume open
\newcommand{\OMEGA}  [0] {\SCAL{\Omega}{}{}}
\newcommand{\OMEGAR} [0] {\SCAL{\Omega}{}{r}}
% Volume closure
\newcommand{\BAROMEGA}  [0] {\SCAL{\TOPBAR{\Omega}}{}{}}
\newcommand{\BAROMEGAR} [0] {\SCAL{\TOPBAR{\Omega}}{}{r}}
% Surface open
\newcommand{\GAMMA}  [0] {\SCAL{\Gamma}{}{}}
\newcommand{\GAMMAR} [0] {\SCAL{\Gamma}{}{r}}
% Surface closure
\newcommand{\BARGAMMA}  [0] {\SCAL{\TOPBAR{\Gamma}}{}{}}
\newcommand{\BARGAMMAR} [0] {\SCAL{\TOPBAR{\Gamma}}{}{r}}

% A-DOMAIN 
% Volume open
\newcommand{\OMEGAA}  [0] {\SCAL{\Omega}{\RM{A}}{}}
\newcommand{\OMEGAAC} [0] {\SCAL{\Omega}{\RM{A_{c}}}{}}
\newcommand{\OMEGAAI} [0] {\SCAL{\Omega}{\RM{A_{i}}}{}}
% Volume closure
\newcommand{\BAROMEGAA}  [0] {\SCAL{\TOPBAR{\Omega}}{\RM{A}}{}}
\newcommand{\BAROMEGAAC} [0] {\SCAL{\TOPBAR{\Omega}}{\RM{A_{c}}}{}}
\newcommand{\BAROMEGAAI} [0] {\SCAL{\TOPBAR{\Omega}}{\RM{A_{i}}}{}}

% H-DOMAIN 
% Volume open
\newcommand{\OMEGAH}   [0] {\SCAL{\Omega}{\RM{H}}{}}
\newcommand{\OMEGAHS}  [0] {\SCAL{\Omega}{\RM{H_{s}}}{}}
\newcommand{\OMEGAHC}  [0] {\SCAL{\Omega}{\RM{H_{c}}}{}}
\newcommand{\OMEGAHR}  [0] {\SCAL{\Omega}{\RM{H}}{r}}
\newcommand{\OMEGAHSR} [0] {\SCAL{\Omega}{\RM{H_{s}}}{r}}
\newcommand{\OMEGAHCR} [0] {\SCAL{\Omega}{\RM{H_{c}}}{r}}
% Volume closure
\newcommand{\BAROMEGAH}   [0] {\SCAL{\TOPBAR{\Omega}}{\RM{H}}{}}
\newcommand{\BAROMEGAHS}  [0] {\SCAL{\TOPBAR{\Omega}}{\RM{H_{s}}}{}}
\newcommand{\BAROMEGAHC}  [0] {\SCAL{\TOPBAR{\Omega}}{\RM{H_{c}}}{}}
\newcommand{\BAROMEGAHR}  [0] {\SCAL{\TOPBAR{\Omega}}{\RM{H}}{r}}
\newcommand{\BAROMEGAHSR} [0] {\SCAL{\TOPBAR{\Omega}}{\RM{H_{s}}}{r}}
\newcommand{\BAROMEGAHCR} [0] {\SCAL{\TOPBAR{\Omega}}{\RM{H_{c}}}{r}}

% HA-INTERFACE 
% Surface open
\newcommand{\GAMMAA}   [0] {\SCAL{\Gamma}{\RM{A}}{}}
\newcommand{\GAMMAH}   [0] {\SCAL{\Gamma}{\RM{H}}{}}
\newcommand{\GAMMAE}   [0] {\SCAL{\Gamma}{\RM{E}}{}}
\newcommand{\GAMMAJ}   [0] {\SCAL{\Gamma}{\RM{J}}{}}
\newcommand{\GAMMAHA}  [0] {\SCAL{\Gamma}{\RM{HA}}{}}
\newcommand{\GAMMAHR}  [0] {\SCAL{\Gamma}{\RM{H}}{r}}
\newcommand{\GAMMAER}  [0] {\SCAL{\Gamma}{\RM{E}}{r}}
\newcommand{\GAMMAJR}  [0] {\SCAL{\Gamma}{\RM{J}}{r}}
\newcommand{\GAMMAHSR} [0] {\SCAL{\Gamma}{\RM{H_{s}}}{r}}
\newcommand{\GAMMAHCR} [0] {\SCAL{\Gamma}{\RM{H_{c}}}{r}}
\newcommand{\GAMMAHAR} [0] {\SCAL{\Gamma}{\RM{{HA}}}{r}}
\newcommand{\GAMMAS}   [0] {\SCAL{\Gamma}{\RM{s}}{}}
\newcommand{\GAMMAC}   [0] {\SCAL{\Gamma}{\RM{c}}{}}
\newcommand{\GAMMAEQ}  [0] {\SCAL{\Gamma}{\RM{eq}}{}}
\newcommand{\GAMMASR}  [0] {\SCAL{\Gamma}{\RM{s}}{r}}
\newcommand{\GAMMACR}  [0] {\SCAL{\Gamma}{\RM{c}}{r}}
\newcommand{\GAMMAEQR} [0] {\SCAL{\Gamma}{\RM{eq}}{r}}
% Surface closure
\newcommand{\BARGAMMAA}   [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{A}}{}}
\newcommand{\BARGAMMAH}   [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{H}}{}}
\newcommand{\BARGAMMAE}   [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{E}}{}}
\newcommand{\BARGAMMAJ}   [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{J}}{}}
\newcommand{\BARGAMMAHA}  [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{{HA}}}{r}}
\newcommand{\BARGAMMAHR}  [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{H}}{r}}
\newcommand{\BARGAMMAER}  [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{E}}{r}}
\newcommand{\BARGAMMAJR}  [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{J}}{r}}
\newcommand{\BARGAMMAHSR} [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{H_{s}}}{r}}
\newcommand{\BARGAMMAHCR} [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{H_{c}}}{r}}
\newcommand{\BARGAMMAHAR} [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{{HA}}}{r}}
\newcommand{\BARGAMMAS}   [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{s}}{}}
\newcommand{\BARGAMMAC}   [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{c}}{}}
\newcommand{\BARGAMMAEQ}  [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{eq}}{}}
\newcommand{\BARGAMMASR}  [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{s}}{r}}
\newcommand{\BARGAMMACR}  [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{c}}{r}}
\newcommand{\BARGAMMAEQR} [0] {\SCAL{\TOPBAR{\Gamma}}{\RM{eq}}{r}}
% Edge open
\newcommand{\ELLHR} [0] {\SCAL{\ell}{\RM{H}}{r}}
\newcommand{\ELLER} [0] {\SCAL{\ell}{\RM{E}}{r}}
\newcommand{\ELLJR} [0] {\SCAL{\ell}{\RM{J}}{r}}
% Edge closure
\newcommand{\BARELLHR} [0] {\SCAL{\TOPBAR{\ell}}{\RM{H}}{r}}
\newcommand{\BARELLER} [0] {\SCAL{\TOPBAR{\ell}}{\RM{E}}{r}}
\newcommand{\BARELLJR} [0] {\SCAL{\TOPBAR{\ell}}{\RM{J}}{r}}

% Unit pointing vectors
\newcommand{\VECNOMEGAR}  [0] {\VEC{n}{\OMEGAR}{}}
\newcommand{\VECNOMEGA}   [0] {\VEC{n}{\OMEGA}{}}
\newcommand{\VECX}        [0] {\VEC{x}{}{}}
\newcommand{\VECY}        [0] {\VEC{y}{}{}}
\newcommand{\VECZ}        [0] {\VEC{z}{}{}}

\newcommand{\VECLR}  [0] {\VEC{l}{}{r}}
\newcommand{\VECMR}  [0] {\VEC{m}{}{r}}
\newcommand{\VECNR}  [0] {\VEC{n}{}{r}}
\newcommand{\SCALLR} [0] {\SCAL{l}{}{r}}
\newcommand{\SCALMR} [0] {\SCAL{m}{}{r}}
\newcommand{\SCALNR} [0] {\SCAL{n}{}{r}}

\newcommand{\VECLGAMMAR}  [0] {\VEC{l}{\Gamma}{r}}
\newcommand{\VECMGAMMAR}  [0] {\VEC{m}{\Gamma}{r}}
\newcommand{\VECNGAMMAR}  [0] {\VEC{n}{\Gamma}{r}}
\newcommand{\SCALLGAMMAR} [0] {\SCAL{l}{\Gamma}{r}}
\newcommand{\SCALMGAMMAR} [0] {\SCAL{m}{\Gamma}{r}}
\newcommand{\SCALNGAMMAR} [0] {\SCAL{n}{\Gamma}{r}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* VARIABLES *************************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Vector fields
\newcommand{\VECA}     [0] {\VEC{A}{}{}}
\newcommand{\VECASTAR} [0] {\VEC{A}{}{\star}}

\newcommand{\VECH}   [0] {\VEC{H}{}{}}
\newcommand{\VECHR}  [0] {\VEC{H}{}{r}}
\newcommand{\VECHTR} [0] {\VEC{H}{\RM{t}}{r}}
\newcommand{\VECHNR} [0] {\VEC{H}{\RM{n}}{r}}

\newcommand{\VECB}   [0] {\VEC{B}{}{}}
\newcommand{\VECJ}   [0] {\VEC{J}{}{}}

\newcommand{\VECE}   [0] {\VEC{E}{}{}}
\newcommand{\VECES}  [0] {\VEC{E}{\RM{s}}{}}
\newcommand{\VECER}  [0] {\VEC{E}{}{r}}

\newcommand{\VECK}   [0] {\VEC{K}{}{}}
\newcommand{\VECKR}  [0] {\VEC{K}{}{r}}
\newcommand{\VECKSR} [0] {\VEC{K}{\RM{s}}{r}}
\newcommand{\VECKCR} [0] {\VEC{K}{\RM{c}}{r}}

\newcommand{\VECCHI}   [0] {\VEC{\boldsymbol{\ITchi}}{}{}}
\newcommand{\VECCHIR}  [0] {\VEC{\boldsymbol{\ITchi}}{}{r}}
\newcommand{\VECCHITR} [0] {\VEC{\boldsymbol{\ITchi}}{\RM{t}}{r}}
\newcommand{\VECCHINR} [0] {\VEC{\boldsymbol{\ITchi}}{\RM{n}}{r}}

% Scalar fields
\newcommand{\SCALT} [0] {\SCAL{T}{}{}}

% vector sources
\newcommand{\MATUS}  [0] {\MAT{u}{s}{}}
\newcommand{\MATIS}  [0] {\MAT{i}{s}{}}
\newcommand{\SCALUR} [0] {\SCAL{u}{}{r}}
\newcommand{\SCALIR} [0] {\SCAL{i}{}{r}}

% basis functions
\newcommand{\BASISVECWI}   [0] {\VEC{w}{i}{}}
\newcommand{\BASISVECWJ}   [0] {\VEC{w}{j}{}}
\newcommand{\BASISVECVP}   [0] {\VEC{v}{p}{}}
\newcommand{\BASISVECVQR}  [0] {\VEC{v}{q}{r}}
\newcommand{\BASISSCALNM}  [0] {\SCAL{N}{m}{}}
\newcommand{\BASISSCALNN}  [0] {\SCAL{N}{n}{}}
\newcommand{\BASISSCALNQR} [0] {\SCAL{N}{q}{r}}

% Discrete fields
\newcommand{\DISCRAJ}  [0] {\SCAL{a}{j}{}}
\newcommand{\DISCRHQR} [0] {\SCAL{h}{q}{r}}
\newcommand{\DISCRTN}  [0] {\SCAL{t}{n}{}}

% Other variables
\newcommand{\SCALLAMBDAR} [0] {\lambda^{r}}
\newcommand{\SCALALPHAR}  [0] {\SCAL{\ITalpha}{}{r}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%* PARAMETERS ************************************%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ECRIT}      [0] {\SCAL{E}{\RM{crit}}{}}
\newcommand{\JCRIT}      [0] {\SCAL{J}{\RM{crit}}{}}
\newcommand{\NPOWLAW}    [0] {\SCAL{n}{}{}}
\newcommand{\NRWINDINGS} [0] {\SCAL{N}{\RM{r}}{}}
\newcommand{\RTHINDEX}   [0] {r\operatorname{-}\RM{th}}

\newcommand{\THICKTAPETR} [0] {\SCAL{\ITdelta}{\RM{t}}{r}}
\newcommand{\THICKTAPESR} [0] {\SCAL{\ITdelta}{\RM{s}}{r}}
\newcommand{\THICKTAPECR} [0] {\SCAL{\ITdelta}{\RM{c}}{r}}


\newcommand{\SCALRHOSURFEQR} [0] {\SCAL{\ITrho}{\GAMMAEQ}{r}}
\newcommand{\SCALRHOSURFSR}  [0] {\SCAL{\ITrho}{\GAMMAS}{r}}
\newcommand{\SCALRHOSURFCR}  [0] {\SCAL{\ITrho}{\GAMMAC}{r}}
